Robust Principles: Architectural Design Principles for Adversarially Robust CNNs

Our research aims to unify existing works' diverging opinions on how architectural components affect the adversarial robustness of CNNs. To accomplish our goal, we synthesize a suite of three generalizable robust architectural design principles: (a) optimal range for depth and width configurations, (b) preferring convolutional over patchify stem stage, and (c) robust residual block design through adopting squeeze and excitation blocks and non-parametric smooth activation functions. Through extensive experiments across a wide spectrum of dataset scales, adversarial training methods, model parameters, and network design spaces, our principles consistently and markedly improve AutoAttack accuracy: 1-3 percentage points (pp) on CIFAR-10 and CIFAR-100, and 4-9 pp on ImageNet. The code is publicly available at https://github.com/poloclub/robust-principles.

==> 405-normalization.tex <==
\subsection{Fewer Normalization Layers}
\label{sec:normalization}

Similar to the analysis in the activation layer, we studied both the \textit{number} and the \textit{function} of normalization layers, motivated by our observations on their strong potential to improve robustness \cite{liu2022convnet,vaswani2017attention}.
For example, ConvNeXt increases the accuracy by reducing two out of three normalization layers in a residual block~\cite{liu2022convnet}.
Similarly, transformers also have fewer normalizations, \eg, a single normalization after the self-attention block and the \ac{mlp} block~\cite{vaswani2017attention}. 
Therefore, 
we experiment with setting the total normalization layers to 3, 2, and 1,
and find the average \ac{pgd} accuracies rise to  30.43\%, 30.83\%, and 29.97\% respectively.
Reducing one normalization layer has the highest average robustness, and we find reducing the first normalization shows the optimal \ac{pgd} accuracy of 31.61\%. 

For normalization function, \ac{bn}~\cite{ioffe2015batch} is commonly used in ConvNets to speed up convergence and reduce overfitting. 
Multiple alternative normalizations are proposed to get rid of the dependence on batch size, \eg, \ac{in}~\cite{ulyanov2016instance} and \ac{ln}~\cite{ba2016layer}.
However, there is no clear consensus on the generalization of these alternatives. 
ConvNeXt slightly increases clean accuracy by substituting \ac{ln} for \ac{bn}. 
Other research found directly substituting \ac{ln} for \ac{bn} in the original ResNet leads to suboptimal performance~\cite{wu2018group}. 
Our adversarial training results show that \ac{bn} is still the optimal normalization function in a residual block. 

